Hierarchical Policy Blending as Inference for Reactive Robot Control

Motion generation in cluttered, dense, and dynamic environments is a central topic in robotics, rendered as a multi-objective decision-making problem. Current approaches trade-off between safety and performance. On the one hand, reactive policies guarantee fast response to environmental changes at the risk of suboptimal behavior. On the other hand, planning-based motion generation provides feasible trajectories, but the high computational cost may limit the control frequency and thus safety. To combine the benefits of reactive policies and planning, we propose a hierarchical motion generation method. Moreover, we adopt probabilistic inference methods to formalize the hierarchical model and stochastic optimization. We realize this approach as a weighted product of stochastic, reactive expert policies, where planning is used to adaptively compute the optimal weights over the task horizon. This stochastic optimization avoids local optima and proposes feasible reactive plans that find paths in cluttered and dense environments. Our extensive experimental study in planar navigation and 6DoF manipulation shows that our proposed hierarchical motion generation method outperforms both myopic reactive controllers and online re-planning methods.

==> sections/acknowledgment.tex <==
\section*{ACKNOWLEDGMENT}


==> sections/related_works.tex <==
\section{RELATED WORK}

% 
\todo[inline]{Relations to Inference as Control}

The neural dynamic policies follow a hierarchical scheme as well \cite{bahl_2020_ndp}. In comparison to our approach, they restrict them self to a class of dynamics. The learn-able policy acts on the parameter space of the dynamics. For training reinforcement learning or imitation learning is employed.


% 
The authors in \cite{yang_2020_multi-expert-learning} proposed a hierarchical control scheme that leverages deep reinforcement learning called \textit{multi-expert learning architecture (MELA)}. They fuse given neural network based experts within the parameter level. The fused expert results from a weighted average of the parameters of the different neural networks. 


% 
\cite{zaki_2022_improperRL} proposed an hierarchical control approach given a set of based controllers. The optimal mixing parameters of the mixture of experts is obtained employing reinforcement learning algorithms. 
 
 
 Blending: 
GPs \cite{tresp_2000_bcm, cao_2014_gpoe, cao_2015_gpoe, deisenroth_2015_dgp, liu_2018_rbcm, cohen_2020_gpe},
PROMPS \cite{paraschos_2018_promp}
